Making Neural Machine Reading Comprehension Faster

This study aims at solving the Machine Reading Comprehension problem where questions have to be answered given a context passage. The challenge is to develop a computationally faster model which will have improved inference time. State of the art in many natural language understanding tasks, BERT model, has been used and knowledge distillation method has been applied to train two smaller models. The developed models are compared with other models which have been developed with the same intention.

==> pages/cover.tex <==

\begin{center}
        
     \begin{Large}  \textbf {MAKING NEURAL MACHINE READING COMPREHENSION FASTER}
	\end{Large}	 
       \vspace{0.5cm}
       
	Submitted by
	\vspace{1.0cm}\break
	\textbf{Debajyoti Chatterjee}
	\break
	(Reg No: 91617007)
	\vspace{1.0cm}\break
	\textit{In partial fulfillment of the requirements for the award of 
Master of Science in Computer Science  with Specialization in Machine Intelligence \vspace{0.5cm}\break
of}
		\break \break
	\includegraphics[width=30mm]{logo/cusat}
	\break
	Cochin University of Science and Technology, Kochi
	\vspace{1.0cm}\break
	Conducted by
	\break \break
	\includegraphics[width=30mm]{logo/iiitmk}\break
	Indian Institute of Information Technology and Management-Kerala\break Technopark Campus\break Thiruvanathapuram-695 581	
	\vspace{0.50cm} \break
	
	April 2019
   \end{center}





==> pages/org.tex <==

\begin{center}
       \vspace*{1cm}
 
       \textbf{ORGANIZATION CERTIFICATE}
 
       \vspace{0.5cm}
       
  \begin{center} To be Issued from company or institute on completion of project. (This is a dummy page)\end{center}


.
             

       
   \end{center}




